Energy-Efficient Low-Power Circuit Techniques for Wireless Energy and Data Transfer in IoT Sensor Nodes

In this paper, we present techniques and examples to reduce power consumption and increase energy efficiency of autonomous Wireless Sensor Nodes (WSNs) for the Internet of Things. We focus on the RF Energy Harvester (RFEH), the data receiver and the transmitter, all of which have a large impact on the device cost, lifetime and functionality. Co-design of the antenna and the electronics is explored to boost the power conversion efficiency of the RF-DC converter. As a proof of principle, a charge pump rectifier is designed, and its measurement results are presented. To boost the rectifier output voltage, a DC-DC converter that employs maximum power point tracking has been designed. A prototype circuit is also presented that can accommodate an input power level range of 1 {\mu}W to 1 mW and offers peak efficiencies of 76.3% and 82% at 1 {\mu}W and 1 mW, respectively. The co-design principle is also used at the receiver side where the antenna-electronics interface is optimized. It is shown how this technique allows improving the noise figure of the Low Noise Amplifier (LNA) without sacrificing power consumption. As a low power alternative to narrow-band wireless transmission, sub-GHz ultra-wideband is proposed. As a proof of principle, the design of a novel low-power sub-GHz Ultra-Wide-Bandwidth (UWB) transmitter which consumes only 0.28 mW is presented. Its working principle is verified by means of circuit simulations and measurements. The low power nature of the transmitter and receiver principles, combined with the power efficient RF-DC converter paves the way towards the continuous operation of a WSN.

==> Data/Section3p1_3p2/Tex/Sec3p1_3p2.tex <==
%\documentclass[journal]{IEEEtran}
%
%\usepackage{algorithmic}
%\usepackage{amsfonts}
%\usepackage[cmex10]{amsmath}
%\usepackage{amssymb}
%\usepackage{array}
%\usepackage{booktabs}
%\usepackage{cite}
%\usepackage{color}
%\usepackage{epsfig}
%\usepackage{eqparbox}
%%\usepackage{fixltx2e}
%\usepackage{fmtcount}
%\usepackage{footmisc}
%\usepackage{footnote}
%\usepackage{graphicx}
%\usepackage{mathrsfs}
%\usepackage{mathtools}
%\usepackage{mdwmath}
%\usepackage{mdwtab}
%\usepackage{mpfnmark}
%\usepackage{multirow}
%\usepackage{nccfoots}
%\usepackage{psfrag}
%\usepackage{setspace}
%\usepackage{stfloats}
%\usepackage{figure}
%\usepackage{tabulary}
%\usepackage{threeparttable}
%\usepackage{url}
%\usepackage[justification=centering]{caption}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
%%\usepackage[retainorgcmds]{IEEEtrantools}
%
%\interdisplaylinepenalty=2500
%
%%\usepackage[caption=false]{caption}
%%\usepackage[font=footnotesize]{subfig}
%
%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi
%
%\hyphenation{op-tical net-works semi-conduc-tor}
%
%\newcommand{\Var}{\mathrm{var}}
%\newcommand{\Exp}{\mathrm{E}}
%\newcommand{\Cov}{\mathrm{cov}}
%\newcommand{\m}{\mathbf}
%\newcommand{\diag}{\operatorname{diag}}
%\newcommand{\trace}{\mbox{\text{Tr}}}
%\newcommand\FT{\ensuremath{\mathcal{F}}}         % Fourier transform
%\newcommand\invFT{\ensuremath{\mathcal{F}^{-1}}} % inverse Fourier transform
%\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
%\newcommand{\parenthnewln}[1]{\right.\\#1&\left.{}}
%\newcommand{\specialcell}[2][c]{%
%  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
%
%\hyphenation{op-tical net-works semi-conduc-tor}
%
%\begin{document}

\subsection{Asynchronous Data Conversion}

IoT sensors may be used to sense slowly-varying signals.
In this case, a level-crossing analog-to-digital converter (LC-ADC) can be applied in order to reduce power consumption \cite{YLi}.
%If such slow signals have long periods of low-frequency variation the LC-ADC is required to hold the comparison window for a long time (hundreds of $\unit{ms}$).
%To overcome this problem, the LC-ADC may be designed to operate in the current domain instead of the charge domain \cite{YLi}.
%
%
%The LC-ADC employs two complementary DACs.
%The first one is the level-crossing DAC, which adjusts the comparison window after each conversion by adding/subtracting current at the input node of the level-crossing detector.
%The second DAC is the calibration DAC, which cancels any DC offset during system reset.
%The residue current is fed to the level-crossing detector, which outputs a pulse in case of a level crossing.
Unlike uniform sampling, the level-transition (LT) and UP/DOWN (U/D) pulse sequences are generated only when the input signal crosses a predefined threshold level as illustrated in Fig.~\ref{LCwave}.
More details on the asynchronous front-end design are provided in \cite{YLi}.

%The ECG readout circuits include two RC oscillators on the chip for generating a synchronous clock signal to calibrate the offset of the two DACs, respectively.
%The oscillators are only enabled for calibration during reset.
%The offset calibration is a typical foreground calibration that is enabled during system startup or manual resetting.
%The entire ECG front-end achieves a measured SNDR of around 48 dB when we apply a 6 mVpp sinusoidal input signal at the input of the LNA.
%The entire ECG readout consumes $8.49 \unit{\mu W}$ from a $1 \unit{V}$ supply.
%More details on the ECG monitoring front-end are provided in~\cite{YLi}.

\begin{figure} 
\centering
\psfig{figure=Data/Section3p1_3p2/figure/LCwave1.eps,width=.9\columnwidth}
\caption{Input and output signals of the level-crossing ADC.}
\label{LCwave}
\end{figure}

The two binary outputs (LT and U/D) must then be both fed to the data transmitter.
They have to be combined and transmitted simultaneously, otherwise information would be lost.
As the transmitter is powered by an RFEH, to minimize power consumption, the data transmission should be only enabled when ADC data conversion is active.
The following subsections present two alternative circuits to transmit the data provided by the asynchronous ADC, one passive and one active circuit.

%The measured low noise amplifier gain and SNDR of the ECG monitoring front-end over frequency are presented in Fig.~\ref{Gain} and Fig.~\ref{sndr}, respectively.
%The plot proves the performance of the ECG front-end with $34 \unit{dB}$ gain from $0.06 \unit{Hz}$ to $950 \unit{Hz}$ and $48 \unit{dB}$ SNDR for an input voltage of $6 \unit{mV}$.
%The LC-ADC has both magnitude resolution and time resolution.
%As time resolution is included in the measurement, the overall SNDR is degraded compared to the stand-alone LNA SNDR.
%
%\begin{figure} 
%\centering
%\psfig{figure=Data/Section3p1_3p2/figure/gainlna.eps,width=.9\columnwidth}
%\caption{Measured gain and bandwidth of the low noise amplifier.}
%\label{Gain}
%\end{figure}
%
%\begin{figure} 
%\centering
%\psfig{figure=Data/Section3p1_3p2/figure/SNDR21.eps,width=.9\columnwidth}
%\caption{Measured total SNDR of the ECG monitoring front-end.}
%\label{sndr}
%\end{figure}


\subsection{Passive Data Transmission }
\label{passive_trasmission}

Employing pulse duration modulation (PDM), the 2-bit data stream is combined to generate pulses with different time duration for upward conversion and downward conversion.
This means that the transmitter produces a pulse when LT indicates a conversion and U/D defines the duration of this pulse.
In this way the 2-bit information can be embedded in a single pulse.
Fig.~\ref{TX} presents the circuit diagram of the transmitter that includes a digital pulse encoder and a backscattering network.
The pulses are generated by comparing LT to $\rm \overline{LT}$, the latter being the complement of LT delayed by six cascaded current starved inverters.
The delay time is set by U/D that makes the pulses longer when it is set to 1.

\begin{figure} 
\centerline{\psfig{figure=Data/Section3p1_3p2/figure/TX1.eps,width=.99\columnwidth}}
\caption{Circuit diagram of the asynchronous transmitter.}
\label{TX}
\end{figure}


The delay is defined by the current drawn in the inverters and capacitor $\rm C_{DL}$. For U/D equal to 1 (upward level crossing) $\rm C_{DL}$ is connected to ground, thus the pulse width is longer.
For U/D equal to 0 (downward level crossing) $\rm C_{DL}$ is disconnected from ground, thus the duration of the pulses is shorter.
Fig.~\ref{TXwave} shows the waveforms of the low-power pulse encoder: the pulse duration is $\rm t_U$ for upward conversion and $\rm t_D$ for downward conversion.


\begin{figure} 
\centering
\psfig{figure=Data/Section3p1_3p2/figure/TX_wave1.eps,width=.8\columnwidth}
\caption{Waveforms of the asynchronous encoder.}
\label{TXwave}
\end{figure}

As an example, we present a circuit designed for backscattering data transmission in which the pulsed signal modulates a $402 \unit{MHz}$ RF signal received in the LC network, implementing  ON-OFF-Keying modulation through transistor $\rm M_0$ (see Fig.~\ref{TX}) \cite{AM1}.
The values of $\rm L_S$ and $\rm C_S$ are 32 nH and 4.9 pF, respectively.
Fig. \ref{Encoder} illustrates the measured waveforms of the asynchronous pulse encoder.
In Fig.~\ref{U0} the output of the pulse encoder is presented for an LT transition with U/D = 0.
In this condition the pulse width is $80 \unit{ns}$. For a LT transition with U/D = 1, the pulse width equals $40 \unit{ns}$, as shown in Fig.~\ref{U1}.


\begin{figure}
\centering
\subfigure[]{
\psfig{figure=Data/Section3p1_3p2/figure/EncodU0.eps,width=0.8\columnwidth}
\label{U0}
}
\subfigure[]{
\psfig{figure=Data/Section3p1_3p2/figure/EncodU1.eps,width=0.8\columnwidth}
\label{U1}
}
\caption{Measured encoder output waveforms: (a) 80 ns or U/D = 0 and (b) 40 ns for U/D = 1.}
\label{Encoder}
\end{figure}


%%\pagebreak
%\begin{thebibliography}{1}
%
%\bibitem{YLi}
%Yongjia Li, Andre L. Mansano, Yuan Yuan, Duan Zhao and Wouter A. Serdijn, ``An ECG Recording Front-End With Continuous-Time Level-Crossing Sampling,'' \textit{IEEE Transactions on Biomedical Circuits and Systems}, Vol.8, No.5, pp.1932-4545, Oct., 2014.
%
%\bibitem{AM1}
%Andre L. Mansano, Yongjia Li, Sumit Bagga and Wouter A. Serdijn, ``An Asynchronous Event-Driven Data Transmitter for Wireless ECG Sensor Nodes,'' \textit{IEEE Biomedical Circuits and Systems Conference}, pp.404-407, Oct., 2014.
%
%
%\end{thebibliography}
%
%\end{document} 


==> Data/Section_4/IoT_4.tex <==
% By contrast, for an LNA with the same circuit
%topology but a $50 \unit{\Omega}$ power-matching interface, $R_{A}$
%and $X_{A}$ cannot be selected freely, and hence the noise
%factor can only be reduced by sacrificing power. Reducing the power
%consumption is the main benefit offered by the proposed co-design
%principle. The input-referred noise of $R_{g}$ is suppressed
%by the interface gain due to the presence of the external capacitor
%$C_{ext}$. This is indicated by $\delta$, which scales
%with $1/Q^{2}$ when $C_{ext}\ensuremath{\gg}C_{gs}$. 




==> Power/Section2p2_2p3/Tex/Sec2p2.tex <==
%\documentclass[journal]{IEEEtran}
%
%\usepackage{algorithmic}
%\usepackage{amsfonts}
%\usepackage[cmex10]{amsmath}
%\usepackage{amssymb}
%\usepackage{array}
%\usepackage{booktabs}
%\usepackage{cite}
%\usepackage{color}
%\usepackage{epsfig}
%\usepackage{eqparbox}
%%\usepackage{fixltx2e}
%\usepackage{fmtcount}
%\usepackage{footmisc}
%\usepackage{footnote}
%\usepackage{graphicx}
%\usepackage{mathrsfs}
%\usepackage{mathtools}
%\usepackage{mdwmath}
%\usepackage{mdwtab}
%\usepackage{mpfnmark}
%\usepackage{multirow}
%\usepackage{nccfoots}
%\usepackage{psfrag}
%\usepackage{setspace}
%\usepackage{stfloats}
%\usepackage{subfigure}
%\usepackage{tabulary}
%\usepackage{threeparttable}
%\usepackage{url}
%\usepackage[justification=centering]{caption}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
%%\usepackage[retainorgcmds]{IEEEtrantools}
%
%\interdisplaylinepenalty=2500

%\usepackage[caption=false]{caption}
%\usepackage[font=footnotesize]{subfig}

\ifCLASSOPTIONcaptionsoff
  \usepackage[nomarkers]{endfloat}
 \let\MYoriglatexcaption\caption
 \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
\fi

\newcommand{\Var}{\mathrm{var}}
\newcommand{\Exp}{\mathrm{E}}
\newcommand{\Cov}{\mathrm{cov}}
\newcommand{\m}{\mathbf}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\mbox{\text{Tr}}}
\newcommand\FT{\ensuremath{\mathcal{F}}}         % Fourier transform
\newcommand\invFT{\ensuremath{\mathcal{F}^{-1}}} % inverse Fourier transform
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\parenthnewln}[1]{\right.\\#1&\left.{}}
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

%\begin{document}


\subsection{Charge Pump Rectifier Topology}

The RF power presented at the rectifier's input must now be converted into DC power, generating a DC output voltage in an efficient manner.
The theoretical model and analysis of the rectifier designed in this work have been first presented in~\cite{AM}.
Fig.~\ref{RFEHBD} shows the block diagram of the designed RFEH that comprises a passive voltage boosting network and an orthogonally switching charge pump rectifier (OS-CPR). The circuit diagram of the boosting network and on-chip OS-CPR are shown in Fig.~\ref{VBN} and Fig.~\ref{OSCPR}.
To adequately drive the OS-CPR, the boosting network delivers large swing control ($\rm V_{b+}$ and $\rm V_{b-}$) and energy signals ($\rm V_{r+}$ and $\rm V_{r-}$). The resonant circuit of the boosting network is modeled by the self-inductance of the antenna, $\rm L_A$, its series resistance, $\rm R_A$, and capacitance $\rm C_{V,T}$ , which is the sum of the on-chip tuning capacitances ($\rm C_D$ and $\rm C_B$) and input capacitance of the rectifier ($\rm C_{R,T}$). An inductive choke $\rm L_C$ provides a DC short at the input terminals of the rectifier to ensure a zero DC offset error at the input of the OS-CPR. In the boosting network design there is a trade-off between the value of $\rm C_{V,T}$ and $\rm L_A$. If $\rm L_A$ is made too large, to increase voltage gain, $\rm C_{V,T}$ has to be very small. In such a case, the resonance frequency will be too sensitive to the rectifier input capacitance that changes with the load and input power. Moreover, increasing the value of $\rm L_A$ requires an inductor that is physically bigger and consequently has a bigger $\rm R_A$, which limits the voltage gain of the boosting network.

The rectifier circuitry (of a single stage) is made up of PMOS transistors as voltage-controlled switches ($\rm M_1$ and $\rm M_2$) and capacitors for AC coupling ($\rm C_C$) and energy storage ($\rm C_{R1}$ and $\rm C_{R2}$) \cite{AM}. 
In order to minimize bulk effects on the threshold voltage, isolated transistors are required.
PMOS transistors are used rather than NMOS because of their intrinsic isolation with the substrate. Isolated NMOS devices are available in the chosen technology but a large area is required due to the deep N-Well and the isolation ring.
Table~\ref{devices} shows the component values of the designed RFEH.

\begin{figure} 
%\captionsetup{justification=centering}
\centerline{\psfig{figure=Power/Section2p2_2p3/figure/EHblock.pdf,width=0.97\columnwidth}}
\caption{\small Block diagram of the RF energy harvester~\cite{AM}.}
\label{RFEHBD}
\end{figure}

\begin{figure}
%\captionsetup{justification=centering}
\begin{center}
\subfigure[]{
\hspace{-1mm}\centerline{\includegraphics[width=0.99\columnwidth]{../figure/VBN.eps}}
\label{VBN}
}
\subfigure[]{
\centerline{\psfig{figure=Power/Section2p2_2p3/figure/OSCPR.eps,width=0.8\columnwidth}}
\label{OSCPR}
}
\end{center}
\caption{Circuit diagram of (a) boosting network and (b) a single stage of the on-chip rectifier in the RFEH~\cite{AM}.}
\label{VBNOSCPR}
\end{figure}
%Fig.~\ref{waveEH} shows the various waveforms in the charge pump rectifier. Each stage has two different DC voltage levels ($\rm V_{CR1}$ and $\rm V_{CR2}$) and AC voltages that are provided by the boosting network.
 Due to DC voltage differences within the stage, the transistors may conduct current in the backward direction in the phase they should be turned off. Known as flow-back current this effect reduces the efficiency of the rectifier. To reduce the flow-back current, capacitors $\rm C_{DC}$ and resistors $\rm R_{DC}$ set the DC voltages $\rm V_{CR1}$ and $\rm V_{CR2}$ at the gate of $\rm M_1$ and $\rm M_2$, respectively, to guarantee that the drain and source potentials are smaller than the gate potential in the off phase.

%\begin{figure}
%\centerline{\psfig{figure=Power/Section2p2_2p3/figure/waveEH.eps,width=0.8\columnwidth}}
%\caption{\small Waveforms of the OS-CPR integrated in the RFEH.}
%\label{waveEH}
%\end{figure}



%\end{document} 


==> Power/Section2p2_2p3/Tex/Sec2p3.tex <==
%\documentclass[journal]{IEEEtran}
%
%\usepackage{algorithmic}
%\usepackage{amsfonts}
%\usepackage[cmex10]{amsmath}
%\usepackage{amssymb}
%\usepackage{array}
%\usepackage{booktabs}
%\usepackage{cite}
%\usepackage{color}
%\usepackage{epsfig}
%\usepackage{eqparbox}
%%\usepackage{fixltx2e}
%\usepackage{fmtcount}
%\usepackage{footmisc}
%\usepackage{footnote}
%\usepackage{graphicx}
%\usepackage{mathrsfs}
%\usepackage{mathtools}
%\usepackage{mdwmath}
%\usepackage{mdwtab}
%\usepackage{mpfnmark}
%\usepackage{multirow}
%\usepackage{nccfoots}
%\usepackage{psfrag}
%\usepackage{setspace}
%\usepackage{stfloats}
%\usepackage{subfigure}
%\usepackage{tabulary}
%\usepackage{threeparttable}
%\usepackage{url}
%\usepackage[justification=centering]{caption}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
%%\usepackage[retainorgcmds]{IEEEtrantools}
%
%\interdisplaylinepenalty=2500
%
%%\usepackage[caption=false]{caption}
%%\usepackage[font=footnotesize]{subfig}
%
%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi

%\hyphenation{op-tical net-works semi-conduc-tor}

%\newcommand{\Var}{\mathrm{var}}
%\newcommand{\Exp}{\mathrm{E}}
%\newcommand{\Cov}{\mathrm{cov}}
%\newcommand{\m}{\mathbf}
%\newcommand{\diag}{\operatorname{diag}}
%\newcommand{\trace}{\mbox{\text{Tr}}}
%\newcommand\FT{\ensuremath{\mathcal{F}}}         % Fourier transform
%\newcommand\invFT{\ensuremath{\mathcal{F}^{-1}}} % inverse Fourier transform
%\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
%\newcommand{\parenthnewln}[1]{\right.\\#1&\left.{}}
%\newcommand{\specialcell}[2][c]{%
%  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
%
%\hyphenation{op-tical net-works semi-conduc-tor}
%\begin{document}


\subsection{Measurement and Analysis of Power Conversion Efficiency}


%This section describes the measurement results of the RF energy harvester.


%\begin{table}
%\footnotesize
%\renewcommand{\arraystretch}{1.5}
%\caption{RFEH Component Values}
%\label{devices3}
%\centering
%\begin{tabular}{c|c||c|c}
%Device & Value & Device & Value \\
%\hline
%$\rm C_B$ & 7.5 pF&$\rm C_{DC}$ &$\rm\simeq$90 fF \\
%\hline
%$\rm C_D$ & 19.5 pF &$\rm R_{DC}$ &350 k$\rm\Omega$ \\
%\hline
%$\rm C_{R,T}$ & $\rm\simeq$17 pF &$\rm C_{R1},C_{R2}$ & 9.7 pF\\
%\hline
%$\rm C_C$ &9 pF &$\rm M_1,M_2$ & 750/0.2\\
%\hline
%\end{tabular}
%\end{table}

One way of increasing the sensitivity is to increase the power conversion efficiency of the RFEH, which is not an easy task since the charge pump rectifier is a non-linear circuit that is sensitive to input power and load variations.

One can see that different PCEs are achieved for different loads and input power levels, which indicates that the design of the RFEH strongly depends both on its output power and on the power received by the antenna. The latter may change due to different coupling factors as a result of variations in distance and/or alignment of antennas.


The RFEH presents a peak PCE that changes with loading conditions. 
The lower the input power is, the lower is the voltage to switch on the transistors of the charge pump rectifier. 
For high input power the transistors may not be completely turned off, which increases flow-back current. 
In addition, the input impedance of the RFEH changes, which degrades matching with the antenna and therefore the power transferred to the load is not optimal.
To partially overcome this issue, the rectifier load can be modulated to some extent by using a DC-DC converter, which will be discussed next.


%\pagebreak
%\begin{thebibliography}{1}
%
%
%
%\bibitem{AM}
%A.~Mansano, S.~Bagga and W.~Serdijn, ``A High Efficiency Orthogonally Switching Passive Charge Pump Rectifier for Energy Harvesters,''
%\textit{IEEE Transaction on Circuits and Systems I}, Vol. 60, No. 7, pp. 1959-1966, July, 2013.


%\end{thebibliography}

%\end{document} 


==> Power/Section_2_1/IoT_2_1.tex <==
%% LyX 2.2.1 created this file.  For more info, see http://www.lyx.org/.
%% Do not edit unless you really know what you are doing.
%\documentclass[twocolumn,journal]{IEEEtran}
%\usepackage[LGR,T1]{fontenc}
%\usepackage[latin9]{inputenc}
%\usepackage{subscript}
%\usepackage[unicode=true,
% bookmarks=true,bookmarksnumbered=true,bookmarksopen=true,bookmarksopenlevel=1,
% breaklinks=false,pdfborder={0 0 0},pdfborderstyle={},backref=false,colorlinks=false]
% {hyperref}
%\hypersetup{pdftitle={Your Title},
% pdfauthor={Your Name},
% pdfpagelayout=OneColumn, pdfnewwindow=true, pdfstartview=XYZ, plainpages=false}
%\usepackage{breakurl}
%
%\makeatletter
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
%\DeclareRobustCommand{\greektext}{%
%  \fontencoding{LGR}\selectfont\def\encodingdefault{LGR}}
%\DeclareRobustCommand{\textgreek}[1]{\leavevmode{\greektext #1}}
%\ProvideTextCommand{\~}{LGR}[1]{\char126#1}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.
%% for subfigures/subtables
%\usepackage[caption=false,font=footnotesize]{subfig}
%
%\makeatother
%
%\begin{document}
%
%\section{Power management}

\subsection{Co-design of antenna and rectifier}
\label{sec:2_1}

To maximize the power transfer from the antenna to the rectifier, their impedances must be matched.
If an IC is directly connected with an off-chip antenna and the length
between them is electrically short, the antenna and the circuitry
can be directly matched without any intermediate stage(s). An optimum
choice of antenna impedance $Z_A$ and load impedance
$Z_L$ allows us to increase the voltage or current at
the antenna load for the same available power at the antenna. As addressed
in \cite{Mark_TCAS2},\emph{ }one needs to design the electronic circuit
for the largest quality factor of $Z_L$ possible and
subsequently co-design the antenna impedance for conjugate matching\emph{.}
This conclusion is a key point that needs to be considered during
a co-design procedure. If $Z_A$ is conjugately matched
with $Z_L$, and the antenna resistance $R_A$
is much smaller than the antenna reactance $X_A$, the
load voltage can be approximated as:
\begin{equation}
\left.V_{L}\right|_{R_{A}\ll X_{A}}\approx\sqrt{2P_{av}}\frac{X_{A}}{\sqrt{R_{A}}},\label{eq:VoutBoost}
\end{equation}
which suggests that the output voltage is passively boosted by the
presence of the antenna reactance, which forms an LC resonator with
the load. Significant improvement of the rectifier input voltage for large values of Q can be achieved
at the expense of bandwidth. This property is exploited in \cite{Mark_JSSC},
where the input voltage of the RF energy harvester is effectively
increased using a high-Q loop antenna. This voltage boost improves the rectifier sensitivity,
meaning that a wireless sensor node with an RF energy harvester can
be operated at a larger distance from the RF energy source. 

In summary, the two conditions that need to be met for an optimum co-design are
as follows. The first condition is to conjugate match the antenna-electronics
interface as this maximizes both the voltage and current at the load.
%The second condition is to determine at which impedance level conjugate
%matching should occur in order to further increase the load voltage
%or current.
The second condition is related to the fact that, since the available input power and the antenna load are fixed, the voltage at the load cannot be increased to an higher value only by means of proper antenna design. Therefore, one should determine at which impedance level conjugate matching should occur in order to further increase the load voltage or current. 
%\end{document}


==> Power/dcdc.tex <==
\textcolor{black}{Several RF energy harvesting systems systems reported in the literature apply DC-DC converters to up-convert the rectifier output \cite{Visser2013,Hsieh2015,Hwang2014}.
When using this approach, the DC-DC converter switching frequency can be designed to be much lower and its amplitude to be higher than that of the RF signal, resulting in a  combined efficiency of a single-stage rectifier and a DC-DC converter that can be higher than that of a rectifier with multiple stages in some cases.}

%This approach is prefered instead of increasing the number of stages of the rectifier, because the DC-DC converter switching frequency is designed to be much lower than the RF signal, so its efficiency can be higher.
The DC-DC converter is then used to charge a battery or a storage capacitor.
Whenever possible, a storage capacitor is preferred due to its cost, small size and longer lifetime.

%\textbf{Importance of presenting an optimum load to the rectifier.}
%\textbf{What happens when the output voltage increases? Show equations of input resistance of the Boost converter (open loop).}
The DC-DC converter must present the optimum load to the rectifier in order to extract the maximum power out of it.
The most straight forward way to boost the rectifier output is to use a boost converter, which most likely will be operating in Discontinuous Conduction Mode (DCM) due to the low load current, limited by the low available power.
However, the average input resistance of the boost converter is dependent on the output voltage:%, as we can see in the equation:
\begin{equation}
R_{in} = \frac{2 L}{D^2 T} \left( 1 - \frac{V_{in}}{V_{out}} \right),
\end{equation}
in which $T$ is the switching \textcolor{black} {period}, $D$ is the duty cycle, $L$ is the inductor value, $V_{in}$ is the rectifier output voltage (input of the DC-DC converter) and $V_{out}$ is the boost converter output voltage.
While charging a storage capacitor, $V_{out}$ will increase every cycle, taking the rectifier load away from its optimal value.
%\textbf{What if we use a Buck-Boost converter in DCM? Show equation of input resistance in this case.}
This problem can be solved by employing a buck-boost converter, which isolates the input from the output while operating in DCM and which presents the following average input resistance \cite{Martins2016}:
\begin{equation}
R_{in} = \frac{2 L}{D^2 T}.
\label{eq:bbcrin}
\end{equation}

%\textbf{Block diagram. Introduce the idea of charging the Supply capacitor.}\
In this work we propose a non-inverting buck-boost converter to operate with an input power ranging from $1 \unit{\mu W}$ to $1 \unit{m W}$, and an input voltage $V_{in}$ ranging from $0.38$ to $1.3 \unit{V}$, respectively.
The core of the converter is formed by switches $S_1$-$S_4$, inductor $L$ and storage capacitor $C_{store}$ as depicted in Fig. \ref{fig:bbconv}.
Ultimately, the goal of the energy harvesting front-end is to charge $C_{store}$, which will then be used to power the sensor node's circuits.
Capacitor $C_{supply}$ stores the energy necessary to operate the energy harvesting circuits, \textcolor{black}{i.e., it provides supply voltage $V_{dd}$ to them}.
The start-up circuit charges capacitor $C_{supply}$.
It consists of a charge pump and a ring oscillator that can operate with $V_{in}$ down to $250 \unit{mV}$.
It is then turned off by the voltage monitor when $C_{store}$ has enough voltage so that the buck-boost converter can operate and charge $C_{store}$ by itself.
When the voltage on $C_{supply}$ reaches its maximum value ($1.8 \unit{V}$) the voltage monitor redirects the switching signal $V_S$ to switch $S_4$ and keeps $S_5$ off, to start charging $C_{store}$.
When $V_{DD}$ drops below $1.2 \unit{V}$, $S_5$ will be switching while $S_4$ will be off and the converter will charge $C_{supply}$.
Capacitor $C_{rec}$ must be large enough so that its voltage ripple due to the inductor current is negligible.
Not depicted in the block diagram are the Zero Current Detection (ZCD) circuit, which switches off $S_5$ or $S_4$ when the inductor current drops to zero, the oscillator and the ON-time generator \cite{Martins2016}.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{Power/fig/bbconv.pdf}
\caption{Buck-boost converter core circuit}
\label{fig:bbconv}
\end{figure}

%\textbf{Trade-offs. Selecting the inductor based on its size. Show its not possible to obtain a high efficiency for a certain range of input power. Introduce selectable switches.}
When the input/output power decreases the converter efficiency reduces and the switching loss becomes one of the dominant energy loss factors \cite{Hu2011}. %starts to get limited by the switching losses.
This loss can be reduced by decreasing the switching frequency and increasing the inductor value, which will increase the size of the device.
\textcolor{black}{Because off-the-shelf inductors with larger inductance are bulky, and in order to keep the system size as small as possible}, in this work we have selected a $220$-$\unit{\mu H}$ power inductor with a parasitic series DC resistance of $21.1 \unit{\Omega}$ (Coilcraft XPL2010-224ML).
The switching loss can be further reduced by using smaller switches, but there exists a trade-off with conduction loss, since the ON resitance of the switch will increase as its width decreases.
When the input/output power increases the conduction loss becomes dominant.
To design a converter that is efficient both at $1 \unit{\mu W}$ and $1 \unit{mW}$ input power, the switches $S_1$-$S_4$ can be configured to operate in either low-power or high-power mode.
Fig. \ref{fig:switches} presents the circuit diagrams of the switches.
The signal $hp$ controls in what mode the switches will operate.
In the low-power mode, only the $M_{LP}$ transistors are switching while the $M_{HP}$ transistors are always turned off.
In the high-power mode, both $M_{LP}$ and $M_{HP}$ are switching.
Therefore, in the low-power mode, the power necessary to drive the switches is reduced and in the high-power mode the switches series resistance is reduced.
Because for low input power the voltage $V_{in}$ is also low, in switch $S_1$ the low-power transistor $M_{LP1}$ is an NMOS.
In switch $S_4$ an extra NMOS is used ($M_{LP4,N}$) in order to increase the efficiency when the output voltage is low.
However, most of the power transfer happens when $V_{out}$ is high ($E = CV^2/2$), so we use only one NMOS and keep the added parasitic capacitance at node $V_{m2}$ low. 
Switch $S_5$ consists of a single transistor, because the charging of $C_{supply}$ is very short and does not have a strong influence on the efficiency.

\begin{figure*}
\centering
\subfigure[]{\includegraphics{Power/fig/s1.pdf}}
\subfigure[]{\includegraphics{Power/fig/s23.pdf}}
\subfigure[]{\includegraphics{Power/fig/s4.pdf}}
\subfigure[]{\includegraphics{Power/fig/s5.pdf}}
\caption{Switches circuit schematics: (a) switch $S_1$, (b) switches $S_2$ and $S_3$, (c) switch $S_4$ and (d) switch $S_5$}
\label{fig:switches}
\end{figure*}

%\textbf{Introduce the idea of switching off blocks when they are not in use.}
%\textbf{Zero current switching. Switching off the blocks is still not enough. Introduce adaptive biasing of the comprators.}
In the ZCD circuit, the voltage at node $V_{m1}$ is compared to the ground voltage to detect when the inductor current crosses zero.
The comparator operates during a brief period after switches $S_1$ and $S_3$ are turned off.
After the current crosses zero, the comparator is switched off again.
This reduces the average power consumption, but it can be further decreased, while maintaining its speed,  by applying dynamic biasing to the comparator \cite{Martins2016}.


The switching frequency of the buck-boost converter can be selected dynamically, so its average input resistance can change (according to (\ref{eq:bbcrin})). %to present the best load to the rectifier. 
\textcolor{black}{Here, the MPPT circuit performs this frequency selection in order to provide the best load to the rectifier.}
%To change this frequency and select the best load to the rectifier is the function of the MPPT circuit. 
















==> Power/mppt.tex <==

%\textbf{Results. Plots. Power consumption of each block.}

Another crucial block that impacts the overall performance of a WSN is the receiver. This challenge is addressed in the next section.

